Zeta Functions and Complex Dimensions of Relative Fractal Drums: Theory, Examples and Applications

In 2009, the first author introduced a new class of zeta functions, called `distance zeta functions', associated with arbitrary compact fractal subsets of Euclidean spaces of arbitrary dimension. It represents a natural, but nontrivial extension of the theory of `geometric zeta functions' of bounded fractal strings. In this memoir, we introduce the class of `relative fractal drums' (or RFDs), which contains the classes of bounded fractal strings and of compact fractal subsets of Euclidean spaces as special cases. Furthermore, the associated (relative) distance zeta functions of RFDs, extend (in a suitable sense) the aforementioned classes of fractal zeta functions. This notion is very general and flexible, enabling us to view practically all of the previously studied aspects of the theory of fractal zeta functions from a unified perspective as well as to go well beyond the previous theory. The abscissa of (absolute) convergence of any relative fractal drum is equal to the relative box dimension of the RFD. We pay particular attention to the question of constructing meromorphic extensions of the distance zeta functions of RFDs, as well as to the construction of transcendentally $\infty$-quasiperiodic RFDs (i.e., roughly, RFDs with infinitely many quasiperiods, all of which are algebraically independent). We also describe a class of RFDs (and, in particular, a new class of bounded sets), called {\em maximal hyperfractals}, such that the critical line of (absolute) convergence consists solely of nonremovable singularities of the associated relative distance zeta functions. Finally, we also describe a class of Minkowski measurable RFDs which possess an infinite sequence of complex dimensions of arbitrary multiplicity $m\ge1$, and even an infinite sequence of essential singularities along the critical line.

==> macro.tex <==
%\usepackage{mathrsfs, amsthm, amsmath}
%\usepackage{amsfonts}

%\usepackage{pict2e}

%\usepackage{multind}
%\makeindex{n}
%\makeindex{a}

%\usepackage[all]{xy}


%%%%%%%%%%%


%\numberwithin{section}{chapter}
%\numberwithin{equation}{section}

%\makeatletter
%\let\c@proposition\c@theorem
%\let\c@corollary\c@theorem
%\let\c@lemma\c@theorem
%\let\c@definition\c@theorem
%\let\c@example\c@theorem
%\let\c@remark\c@theorem
%\let\c@problem\c@theorem
%\makeatother

%%%%%%%%%%%

%\usepackage{amsthm} % http://tex.stackexchange.com/questions/88721/defining-shared-counters-for-theorem-environments-after-environments-are-defin

%\newtheorem{cor}[theorem]{Corollary}
%\newtheorem{prop}[theorem]{Proposition}

%\theoremstyle{definition}
%\newtheorem{defn}[theorem]{Definition}

%\spnewtheorem{example}[theorem]{Example}






\let\text=\mbox

\catcode`\@=11
\let\ced=\c
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
%\renewcommand{\c}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\g}{\lambda}
\renewcommand{\o}{\omega}
\newcommand{\q}{\quad}
\newcommand{\n}{\nabla}
\newcommand{\s}{\sigma}
\newcommand{\Z}{\mathrm{Z}}
\newcommand{\z}{\zeta}
%\newcommand{\div}{\mathop{\rm div}}
\newcommand{\sing}{{\rm Sing}\,}
%\newcommand{\singg}{{\rm Sing}_\ty\,}

%\newcommand{\cal}{\mathcal}
\newcommand{\Be}{\mathcal{B}}

%\newcommand{\A}{{\cal A}}
%\newcommand{\F}{{\cal F}}
%\newcommand{\H}{{\cal H}}
%\newcommand{\W}{{\bf W}}
\newcommand{\M}{{\cal M}}
%\newcommand{\N}{{\cal N}}
%\newcommand{\S{{\cal S}}


\newcommand{\ty}{\infty}
\newcommand{\e}{\varepsilon}
\newcommand{\f}{\varphi}
%\newcommand{\:}{{\penalty10000\hbox{\kern1mm\rm:\kern1mm}\penalty10000}}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\DD}{\Delta}
\renewcommand{\O}{\Omega}
\newcommand{\pa}{\partial}
\newcommand{\I}{\mathbbm{i}}
\newcommand{\D}{\mathrm{d}}

\newcommand{\st}{\subset}
\newcommand{\stq}{\subseteq}
\newcommand{\pd}[2]{\frac{\pa#1}{\pa#2}}
\newcommand{\pdd}[2]{\frac{\pa^2#1}{\pa#2^2}}
\newcommand{\sgn}{{\rm sgn}\,}
%\newcommand{\sp}[2]{\langle#1,#2\rangle}

\newcount\br@j
\br@j=0
%\newcommand{\q}{\quad}
%\newcommand{\gg}[2]{\hat G_{#1}#2(x)}
%\newcommand{\inty{\int_0^{\ty}}
%\newcommand{\remark{\bigskip\advance\br@j by1 \noindent{\csc Remark
%\the\br@j.}\kern3mm\relax}
\newcommand{\od}[2]{\frac{\D #1}{\D #2}}
\newcommand{\odd}[2]{\frac{\D^2#1}{\D #2^2}}

%\newcommand{\bg}{\begin}
%\newcommand{\eq}{equation}
%\newcommand{\bgeq}{\bg{\eq}}
%\newcommand{\endeq}{\end{\eq}}
%\newcommand{\bgeqnn}{\bg{eqnarray*}}
%\newcommand{\endeqnn}{\end{eqnarray*}}
%\newcommand{\bgeqn}{\bg{eqnarray}}
%\newcommand{\endeqn}{\end{eqnarray}}

%\newcommand{\bgeqq}[2]{\bgeqn\label{#1} #2\left\{\begin{array}{ll}}
%\newcommand{\endeqq}{\end{array}\right.\end{eqnarray}}


%\newcommand{\abstract}{\bgroup\leftskip=2\parindent\rightskip=2\parindent
%        \noindent{\bf Abstract.\enspace}}
%\newcommand{\endabstract{\par\egroup}



\newcommand{\udesno}[1]{\unskip\nobreak\hfil\penalty50\hskip1em\hbox{}
             \nobreak\hfil{#1\unskip\ignorespaces}
                 \parfillskip=\z@ \finalhyphendemerits=\z@\par
                 \parfillskip=0pt plus 1fil}
\catcode`\@=11



\newcommand{\eR}{\mathbb{R}}
\newcommand{\eN}{\mathbb{N}}
\newcommand{\Ze}{\mathbb{Z}}
\newcommand{\Qu}{\mathbb{Q}}
\newcommand{\Ce}{\mathbb{C}}
\newcommand{\Ha}{\mathbb{H}}

%\newcommand{\Re}{\mathop{\mathrm{Re}}}
%\newcommand{\Im}{\mathop{\mathrm{Im}}}
\newcommand{\re}{\mathop{\mathrm{Re}}}
\newcommand{\im}{\mathop{\mathrm{Im}}}
%\newcommand{\mathcal L}{{\mathcal L}}

\newcommand{\sign}{\mathop{\mathrm sign}}


\newcommand{\po}{{\mathop{\mathcal P}}}
\newcommand{\conv}{\mathop{\mathrm conv}}

\newcommand{\sdim}{\mbox{\rm s-dim}\,}
\newcommand{\usdim}{\mbox{s-$\ov\dim$}\,}
\newcommand{\esing}{\mbox{\rm e-Sing}\,}

\newcommand{\res}{\operatorname{res}}
\newcommand{\el}{\mathrm{l}}
\newcommand{\supp}{\operatorname{supp}\,}
%\newcommand{\cal}{\mathcal}

%\advance\baselineskip by 6pt

\newcommand{\sideremark}[1]{\ifvmode\leavevmode\fi\vadjust{\vbox to0pt{\vss % the remark
      \hbox to 0pt{\hskip\hsize\hskip1em           %                will appear only
 \vbox{\hsize2cm\tiny\raggedright\pretolerance10000%                on the side
 \noindent #1\hfill}\hss}\vbox to8pt{\vfil}\vss}}}%
                                                   %                in 3cm

                                                   %                wide box
                                                   %

\newcommand{\edz}[1]{\sideremark{#1}}


\newcommand{\abs}[1]{\lvert#1\rvert}

\newcommand{\osc}{\mathop{\rm osc}}
\newcommand{\avM}{\tilde{\mathcal {M}}}

\newcommand{\qs}{\q}

